RAG-Modulo: Solving Sequential Tasks using Experience, Critics, and Language Models

Large language models (LLMs) have recently emerged as promising tools for solving challenging robotic tasks, even in the presence of action and observation uncertainties. Recent LLM-based decision-making methods (also referred to as LLM-based agents), when paired with appropriate critics, have demonstrated potential in solving complex, long-horizon tasks with relatively few interactions. However, most existing LLM-based agents lack the ability to retain and learn from past interactions - an essential trait of learning-based robotic systems. We propose RAG-Modulo, a framework that enhances LLM-based agents with a memory of past interactions and incorporates critics to evaluate the agents' decisions. The memory component allows the agent to automatically retrieve and incorporate relevant past experiences as in-context examples, providing context-aware feedback for more informed decision-making. Further by updating its memory, the agent improves its performance over time, thereby exhibiting learning. Through experiments in the challenging BabyAI and AlfWorld domains, we demonstrate significant improvements in task success rates and efficiency, showing that the proposed RAG-Modulo framework outperforms state-of-the-art baselines.

==> text/background.tex <==
\section{Background}
In this section, we present the problem of interest.

\subsection{POMDP}
We consider a goal-augmented Partially Observable Markovian Decision Process $(\mathbb{S}, \mathbb{G}, \mathbb{A}, \mathrm{T}, \Omega, \mathbb{O}, \mathrm{R},   \gamma)$ \cite{} in a textual RL environment with a vocabulary $\mathbb{V}$, where $\mathbb{S}$ and $\mathbb{A}$ represents the state and action space. $\mathbb{G}\subset \mathbb{V}^{N}$ represents the goal space comprising of task descriptions. For every action taken $a\in\mathbb{A}$, the environment transitions to the next state $s'\in \mathbb{S}$ using the transition model $\mathrm{T}(s'|s,a)$. The agent can only partially observe the environment, where the observation $o\in \mathbb{O}$ is given by the observation model $\Omega(o|s',a)$. For a given goal $g\in \mathbb{G}$ environment returns the reward $r$ using the function $\mathrm{R}(g,s,a)$. The objective is to learn a policy $\pi:\mathbb{G}\times \mathbb{O}\mapsto \mathbb{A}$ that maximizes the expected sum of discounted future rewards $\mathbb{E}[\sum_{t=0}^H\gamma^t r_t]$, where $H$ and $\gamma$ represents the task horizon and discount factor respectively.


% For every environment state $s\in \mathrm{S}$, an agent observes its textual description $o \in \mathrm{O} \subset \mathbb{V}^{N}$ determined using the observation function $h:\mathrm{S}\mapsto \mathrm{O}$ and takes action $a\in\mathrm{A}\subset \mathbb{V}^{N}$ towards achieving the goal $g\in\mathrm{G}\subset \mathbb{V}^{N}$. The environment returns the reward $r$ using the reward function $\mathrm{f_R}:\mathrm{S}\times\mathrm{A}\times\mathrm{G}\mapsto \mathbb{R}$ and transitions to the next state $s'$ using the transition function $\mathrm{f_T}:\mathrm{S}\times \mathrm{A}\mapsto \mathrm{S}$. 


% \textbf{Hierarchical planning:} In this paper, we consider hierarchical model for planning \cite{sutton1999between}. The model consists of a high-level policy $\pi^H$ that decomposes the goal $g$ into a sequence of sub-goals, each associated with a high-level action $a^H \in \mathrm{A}^H \subset \mathbb{V}^N$ and object(s) visible in the environment. The high-level actions are translated to a sequence of primitive actions $a^L \in \mathrm{A}$ by a low-level policy $\pi^L$ that are executable in the embodied environment. We assume a fixed oracle low-level policy that is either known or pre-trained using synthetic data.

% For example, in AlfWorld, the high-level action space includes actions like \textsc{goto}, \textsc{heat}, \textsc{clean}, \textsc{take} etc. The low-level action primitives consist of navigational commands such as \textsc{MOVE AHEAD}, \textsc{ROTATE LEFT/RIGHT}, and \textsc{LOOK UP/DOWN}, as well as manipulative actions like \textsc{PICKUP}, \textsc{PUT}, \textsc{OPEN}, \textsc{CLOSE}, and \textsc{TOGGLE ON/OFF}. The full list of actions for AlfWorld and BabyAI can be found in the appendix.

\subsection{Hierarchical Planning} 
Hierarchical planning employs an options framework \cite{sutton1999between, daniel2016probabilistic} to break tasks into manageable sub-tasks, accomplish them individually, and then combine them to achieve the overall objective. Each option $c \in \mathbb{C}$ is a temporally extended action, where $\mathbb{C} \subset \mathbb{V}^N$ represents the set of high-level actions, such as "go to a location" or "heat an object." The high-level policy $\pi_H$ selects an option, while the low-level policy $\pi_c$ executes primitive actions $a \in \mathbb{A}$ until a termination condition $\beta_c$ is met. We assume that $(\pi_c, \beta_c)$ are fixed and known.


\subsection{Language Models as Planners} 
In this framework, the high-level policy $\pi_H$ is implemented as a language model that predicts the next option based on a structured prompt. 
\begin{align*}
    \pi_H(c_t) = LM({prompt}_t)
\end{align*}
where, the prompt consists of (i) in-context examples, $\{g^k, o^k, c^k\}_{k=1}^K$, (ii) the history, $(g, o_{1:t-1}, c_{1:t-1})$ and (iii) the current observation, $o_t$. The in-context examples demonstrate how to solve similar tasks and the history of past interactions provides the language model with context about how the agent has interacted with the environment so far. The objective for the model is to generate a plan $\{c_1, c_2, \ldots, c_H\}$ that achieves the given goal $g$.


% \begin{itemize}
%     \item \textbf{LLM}: The language model acts as a high-level agent suggesting a high-level skill to exercise from a pre-defined set of skills $s \in \{1, \ldots, S\}$ based on the policy $\pi^H$.
%     \item \textbf{Agent}: The low-level agent is represented as a collection of fixed low-level policies $\{\pi_s^L\}_{s=1}^S$ and their corresponding termination conditions $\{\beta_s\}$ such that for every high-level skill $s$ suggested by the LLM, the low-level agent exercises the low-level policy $\pi_s^L$ until its terminal condition is met $\beta_s=1$. 
%     \item \textbf{Bank}: The bank holds interactions of LLM with the environment via the low-level agent. The maximum number of interactions that the bank can hold is $|\mathcal{B}|$.
%     \item \textbf{Sample Interaction}: A sample interaction that the bank holds can be represented with the tuple $(i_t, a_t)$ where $i_t = (m, s_t, a_{1:t-1}, f_{t-1}, r_{t-1})$ is the state of the LLM, $m$ is the mission in natural language, $s_t$ is the environment state, $a_{1:t-1}$ is the action history, $f_{t-1} \in \{\textrm{feasible}, \textrm{infeasible}\}$ indicates the feasibility of the last action $a_{t-1}$ and $r_{t-1}$ providing the corresponding reason for infeasibility in natural language.
% \end{itemize}


==> text/introduction_outline_vaibhav.tex <==
\section{INTRODUCTION}



\blue{Hi Abhinav, I am adding my prompts and comments in blue.}


\blue{Introduce the problem of solving long-horizon tasks, given a language-based mission. Discuss why this problem is challenging to solve using RL? Sparse reward, partial observability, ...}

Insert text here...

\blue{Discuss recent success of LLMs in tackling this problem, over planning, reinforcement learning, alone. Planning requires models, which may not be present. RL requires lots of exploratory interaction, which may not be safe or feasible. Discuss what makes LLMs attractive as planners. They typically perform dynamic replaning to increase success.}
\begin{itemize}
    \item \textit{Why dynamic planning?} In partially observable environments, it is difficult to suggest the correct plan in one go from the initial state.  If incorrect, verifying the complete plan while localising the mistake post hoc could be expensive. Some works use plans as programs with if-else conditioning for robust planning but still there is no correctness guarantees. Limited grounding to the current state, which could be bad in partially observable environments with many unexplored areas.
\end{itemize}

\blue{LLMs while attractive and a very active area of research are not the final word on planning. They have limitations. For isntance, one limitations is lack of ability to critic. Cite Rao's papers here. Hence, recently, LLM-Modulo frameworks have been proposed that utilize external critics to improve upon planning.}

 \textit{LLM-Modulo: Why external critics with feasibility feedback?} 

    - While language models have shown to improve their performance with chain-of-thought-prompting \cite{}, they often hallucinate \cite{} and are not inherently equipped for reasoning or planning by themselves \cite{}. However, they excel when working in tandem with formal systems that can handle the logical aspects of planning \cite{}. In LLM-Modulo frameworks, LLMs serve as planners, while a bank of specialized external critics evaluates their decisions based on various criteria, such as correctness, executability, and user preferences. In this paper, we consider such a framework that aims to enhance LLM's decision-making by informing it of past successes and failures via an interactive feedback loop.
    
    - By representing plans as Python programs, we can constrain and verify if any of the constraints are violated, and provide feedback.  This is akin to how programmers also receive the feedback (Compilation Error/Runtime Error) from the compiler for debugging.
     
     - Invoking the critics at each step to learn if the action taken was right or wrong based on different criteria: syntax, semantics and excitability. 
     Syntax Parser: Ensures that the response generated by the LLM conforms to the syntactic rules of the defined options and environment objects. 
     Semantics Parser: Checks that the predicted action is meaningful and logically consistent with the current state of the environment (e.g., if the agent has the key before opening a door). 
     Low-Level Policy Critic: Executes the predicted high-level action and checks if it can be completed (for example obstacle encountered). 
Each critic returns feedback based on its evaluation criteria, and the combined feedback determines whether the predicted action is feasible or not. This feedback is passed back to the LLM, enabling it to refine its next prediction.

\blue{Informed by this active area of work in LLM-assisted planning, we identify anotherh challenge: the lack of learning in LLM agents. While RL agents are able to learn over time by storing past interactions (replay buffer). LLM agents typically do not leverage past interactions. Skills are used as a proxy for memory. Cite Boss, Voyager, etc. here. But not at the level of interactions. This is an importatnt limitaiton for robotics applications, in which learning is critical. Another approach is asking human users to refine the prompt. This is also not scalable.}
Insert text here...

\blue{In this work, we consider the problem of leraning with LLM agents based on past interactions. One approach is to fine-tune the foundation model. however, this is expensive and not possible for closed-source model. It is also not scalable in terms of computational cost, resources, and efficiency.}
Insert text here...


\blue{Hence, we propose the idea of using interactio as a memory. Describe our idea: past interactions are stored in a database. This can be derived through environmental interaction or experts. Then, analogous to RAG, context-specific interactions are retrieved when a new planning problem. This enables automatic tuning of prompt for new planning problems. To our knowledge, this work is the first to ....}


    \textit{Why RAG system?} The bank of interactions encompass past mistakes and rectifications. Leveraging the bank should allow the agent to generalize from past experiences, avoid mistakes previously encountered and drive towards correct decision-making. This is similar to how humans recall and learn from their own mistakes.  
    
    Also, the previous two aspects alone would be costly if non-ergodic states were to be present in the environment, since low-level agent won't be able to recover. RAG system can be used to recall such costly mistakes from the past and avoid them in future. 
    

\blue{Building on this key insight, we make three contributions. 
(1) XYZ: An LLM-based planner that builds on LLM Modulo framework to include interaction memory (2) A retrieval mechanism that enables LLM Modulo agents to retrieve context-aware interactions from its memory and automatically tune its prompts, thereby reducing the manual effort required to tune prompts (3) A suite of experiments on challenging planing tasks (AlfWorld and Minigrid) where XYZ outperforms recent baselines and demonstrates improvement in performance with more number of interactions. We argue that \approach should have two key-components: real-time feasibility feedback and stored memories in order to more informed and adaptive decision-making.}

Our approach: Use LLM as candidate planners in an LLM-Modulo framework where 
\begin{itemize}
    \item the LLM iteratively specifies the sequence of sub-tasks to complete to achieve the overarching objective
    \item Before proceeding to the next sub-task, the feasibility of the previous one is checked by an external agent and communicated back to the LLM via back-prompting
    \item At each step, the sample plan is updated with the interactions most relevant to the current state using a RAG system
\end{itemize}


==> text/old_introduction.tex <==
\section{Introduction}

% Long-horizon tasks are difficult to solve because they require the agent to complete multiple sub-tasks \cite{?}. Traditional reinforcement learning algorithms often struggle in these environments due to sparse rewards \cite{?}. This challenge is further intensified in partially observable environments, where the agent must engage in exploratory interactions, which may not always be safe or feasible \cite{?}.

% Chris - A lot of people want to build LLM-based agents that can interact with their environment to solve interactive, real-world problems.  A desirable property for any approach to solving interactive tasks is that the agent get better over time, as it has more experience interacting with its environment.  The classic approach to this would be deep reinforcement learning. But the problem with an LLM-based agent is that training or even fine-tuning an LLM through RL is not reasonable in most cases.  The best LLMs are closed-source, and even large open-source models take an unreasonable amount of resources (CPU, RAM, episodes) to train.  Thus, we propose a framework for deploying LLM-based agents that learns not through back-propagation, but by building up a database of experiences that it then accesses by simply issuing queries.  We show that this approach effectively allows for learning-by-doing, but at a fraction of the cost of 
% back-propagation.

Language models have emerged as promising tools for planning in long-horizon tasks. They can approximate world knowledge \cite{?} and, with few-shot reasoning, decompose high-level tasks into mid-level plans without any further training \cite{?}. Additionally, they can serve as dynamic planners, adapting their strategies in response to environmental feedback in partially observable settings, improving the likelihood of successful task completion \cite{?}.

Despite their recent success, language models face two key challenges. First, they often hallucinate \cite{} and are not inherently designed for reasoning or planning on their own \cite{}. However, they have demonstrated strong performance when integrated with formal systems capable of handling the logical aspects of planning \cite{}. In LLM-Modulo frameworks, language models act as planners, while a bank of specialized external critics evaluates their decisions based on criteria such as correctness, executability, and user preferences. In this paper, we explore a framework that aims to enhance LLM decision-making by incorporating feedback from these critics.


Second, LLM agents lack memory of past interactions. While reinforcement learning agents can learn over time by storing interactions in a replay buffer, LLM-based agents typically do not leverage such memory \cite{?}. A common solution involves providing in-context examples to the LLM, but this approach is limited by the selection of examples and is not scalable. Another approach is to fine-tune language models on past interactions \cite{}, but this can be computationally expensive and resource-intensive. Recent work has explored storing high-level abstractions of past interactions, often referred to as skills, in memory \cite{}. However, these systems are designed to recall interactions at the skill level, potentially losing crucial details about past mistakes and their corrections scattered across the memory database. 
To address both challenges, we propose \approach, which enhances LLM decision-making by incorporating past successes and failures through an interactive feedback loop. First, we invoke a bank of critics at each step of the generation process to assess the feasibility of the action based on criteria such as syntax, semantics, and executability. By representing plans as Python programs \cite{?}, syntactic feedback ensures that the LLM's response adheres to the grammar rules of the environment. Semantic feedback verifies that the predicted action is meaningful and logically consistent with the current state (e.g., ensuring the agent has a key before attempting to open a door). The low-level policy critic executes the predicted high-level action and checks for completion (e.g., determining if an obstacle is encountered). This process is similar to how programmers receive feedback (e.g., Compilation Error/Runtime Error) from compilers during debugging.

Second, we store these interactions, along with their feasibility feedback, in a database. Similar to Retrieval-Augmented Generation \cite{?}, context-aware interactions are retrieved as in-context examples when encountering new planning problems. This enables automatic prompt tuning for new tasks. By leveraging these past interactions, the agent can generalize from previous experiences, avoid recurring mistakes, and make more accurate decisions, akin to how humans learn from their own errors.

Building on this insight, we make the following contributions: 
\begin{itemize} 
    \item \approach: An LLM-based planner that extends the LLM Modulo framework by incorporating interaction memory. 
    \item A retrieval mechanism that enables LLM Modulo agents to access context-aware interactions from memory as in-context examples, automatically tuning prompts and reducing manual effort. 
    \item A suite of experiments on challenging planning tasks from AlfWorld and Baby Minigrid, where \approach outperforms recent baselines and demonstrates improved performance with minimal environment interactions. We argue that \approach should have two key-components: real-time feasibility feedback and stored memories in order to more informed and adaptive decision-making.
\end{itemize}


